A Survey of Automatic Evaluation Methods on Text, Visual and Speech Generations

Recent advances in deep learning have significantly enhanced generative AI capabilities across text, images, and audio. However, automatically evaluating the quality of these generated outputs presents ongoing challenges. Although numerous automatic evaluation methods exist, current research lacks a systematic framework that comprehensively organizes these methods across text, visual, and audio modalities. To address this issue, we present a comprehensive review and a unified taxonomy of automatic evaluation methods for generated content across all three modalities; We identify five fundamental paradigms that characterize existing evaluation approaches across these domains. Our analysis begins by examining evaluation methods for text generation, where techniques are most mature. We then extend this framework to image and audio generation, demonstrating its broad applicability. Finally, we discuss promising directions for future research in cross-modal evaluation methodologies.

==> sections/AE/ae_nlg_subsections/backup.tex <==
\section{Automatic Evaluation for NLG}

In this section, we comprehensively investigate the progress of the automatic evaluation techniques in the NLG tasks, such as dialogue generation, summarization, translation and \textit{etc.}. 

The structure of this section is organized as follows: 
(1) We first propose the taxonomy framework in Section~\ref{sec:taxonomy_nlg}, investigating the four major technique paradigms shift in automatic evaluation techniques; 
(2) We then compile the widely used and meta-evaluation benchmarks in Section~\ref{sec:meta_evaluation_benchmarks} that are used to evaluate the effectiveness of the automatic evaluation metrics;
(3) We summarize the features of these methods and answer some open problems in Section~\ref{sec:conclusion_challenge_future}.

\subsection{Taxonomy}
\label{sec:taxonomy_nlg}

%\input{sections/figure_taxonomy}
\input{sections/table_eval_metric}


As shown in Figure~\ref{}, existing automatic evaluation methods for NLG could be classified into five categories: \textbf{\textcircled{\scriptsize{1}}} \textbf{\textit{Heuristic evaluation}:} Early automatic evaluation, which primarily focus on leveraging rule-based and heuristic features in text modal, such as word-overlap or generation probabilities;
\textbf{\textcircled{\scriptsize{2}}} \textbf{\textit{Embedding-based Evaluation}:} With the rapid development of the distributed word embeddings and representation learning~\cite{10007404,pennington-etal-2014-glove,devlin-etal-2019-bert}, numeous works measures the semantic similarity between references and generations~\cite{zhang2020bertscoreevaluatingtextgeneration};
\textbf{\textcircled{\scriptsize{3}}} \textbf{\textit{Learning-based Evaluation}:} As the scale of human-annotated evaluation data gradually increases, using neural networks to fit human-annotated data have also made tremendous progress;
\textbf{\textcircled{\scriptsize{4}}} \textbf{\textit{LLM-based Evaluation}:} Recently, the strong generalization of large-scale language models (LLMs) promotes researchers to implement flexible and reliable automatic evaluation methods by simply designing the prompts for evaluation, resulting in the, which is also known as the concept of LLM-as-a-judge~\cite{li2024generationjudgmentopportunitieschallenges};
\textbf{\textcircled{\scriptsize{5}}} \textbf{\textit{Benchmark Evaluation}:} As a special form of evaluation, assessing specific capabilities on human-annotated benchmarks, such as mathematical and code reasoning capabilities, is also a common automatic evaluation approach, which we named.

The following content of this subsection delves into a detailed exploration of these categories, each accompanied by their corresponding representative works.

\subsubsection{Heuristic Evaluation}



Heuristic evaluation commonly relies on the rule-based or heuristic features for evaluation, such as word-overlap, edit-distance, and generation Probability. Meanwhile, some works utilize other heuristic information that does not belong to these three categories, which we categorize as ``others''. The complete overview of heuristic evaluation methods are shown in Table~\ref{tab:auto_metric_adoption}.

\paragraph{Word-overlap-based} To the best of our knowledge, most existing word-overlap-based heuristic metrics evaluate text generation from two criteria: (1) text similarity; and (2) text diversity.

\textbf{Text Similarity:} Most metrics assume that generated texts with a high text similarity to the ground truth are of high quality~\cite{ren2020codebleu,hardy-etal-2019-highres,dhingra-etal-2019-handling}.
For example, BLEU~\cite{papineni-etal-2002-bleu} and ROUGE~\cite{lin-2004-rouge} are the most representative metrics, measuring machine translation and text summarization by computing the precision and recall of $n$-grams word-overlap.
Subsequently, numerous word-overlap-based evaluation methods have been proposed to improve these two metrics.
For example, chrF~\cite{popovic-2015-chrf} and METEOR~\cite{banerjee-lavie-2005-meteor} combines precision and recall in $n$-gram matching, thereby providing a more accurate assessment of textual similarity.
NIST~\cite{10.5555/1289189.1289273} and CIDEr~\cite{vedantam2015ciderconsensusbasedimagedescription} computes the weight for different $n$-grams, focusing on crucial important words.
EmbeddingROUGE~\cite{10007404} improves the accuracy of word overlap matching by utilizing semantic similarity measurements based on word2vec vectors~\cite{mikolov2013efficientestimationwordrepresentations}, addressing the drawback of inaccurate text matching.

\textbf{Diversity:} Rep-$n$ and Distinct-$N$ are the most widely used metrics~\cite{su2023contrastive,lan2022momentum,li2023repetition}, computing the ratio of unique $n$-grams in model-generated text. 
Moreover, Self-BLEU~\cite{zhu2018texygenbenchmarkingplatformtext} calculates BLEU score for every generated sentence, and define the average BLEU score to measure the diversity of the generations.
To address the bias for the longer generations of Distinct-$N$, Expectation-Adjusted Distinct (EAD)~\cite{liu-etal-2022-rethinking} scales the number of distinct tokens based on their expectations.

%%%%% fanshu, 补充一致性/QA相关的评估方法

\paragraph{Edit-Distance-based}

Except for computing the word-overlap, numerous works also evaluate the quality of text by computing the edit distance between the generated text and reference answers\textemdash the number of character or word level transformations required to convert the generations into the reference text.
For example, Levenshtein distance~\cite{moramarco-etal-2022-human}, TER~\cite{snover-etal-2006-study} and WER~\cite{negri-etal-2014-quality} evaluate the quality of model-generated summary and translation by computing the edit distance between ground-truth.

\paragraph{Probability-based}

Most previous works notice that there is a positive correlation between the quality of the text and its generation probability~\cite{moon-etal-2022-evaluating,ke-etal-2022-ctrleval,su2023contrastive}.
Therefore, numerous works compute the generation probability or perplexity (ppl) \cite{Jelinek1977PerplexityaMO} for measuring the fluency of generation, using pre-trained language models, such as GPT-2 \cite{radford2019language} and BERT \cite{devlin-etal-2019-bert}.%\footnote{\url{https://huggingface.co/spaces/evaluate-metric/perplexity.}}
For example, BARTScore~\cite{yuan2021bartscoreevaluatinggeneratedtext}, T5Score~\cite{qin2022t5scorediscriminativefinetuninggenerative} measures the generation probability given the input or reference.\footnote{An increasing number of studies utilize extensively and deeply pre-trained LLMs to evaluate the probability of generated text~\cite{li-etal-2024-leveraging-large}, such as GPTScore~\cite{fu2023gptscoreevaluatedesire}. However, since these methods employ large language models, we collectively discuss them under the LLM-based evaluation paradigm (Section~\ref{sec:llm_based_evaluation}). This paragraph primarily focuses on methods that use small-scale pre-trained language models like BERT to evaluate generation probability in the pre-LLM era.}


\paragraph{Others}
In addition to heuristic features based on word-overlap, edit distance, and generation probability, there are also some works leveraging interesting heuristic features for evaluating~\cite{han-etal-2022-measuring,islam-magnani-2021-end,pratapa-etal-2021-evaluating}.
For example, FACE~\cite{NEURIPS2023_37094fdc} measures the text similarity based on Fourier Analysis of the estimated Cross-Entropy of text. ME~\cite{mordido-meinel-2020-mark} proposes a family of evaluation methods inspired from popular population size estimators that have been widely used in ecology.


\subsubsection{Embedding-based Evaluation}
Most heuristic evaluation neglect semantic features in generations, leading to the significant discrepancy with human evaluation. With the rapid development of the distributed word embeddings and representation learning~\cite{10007404,pennington-etal-2014-glove}, \textbf{\textcircled{\scriptsize{2}}} \textbf{\textit{Embedding-based Evaluation}} begins to emerge, which measures the semantic similarity of embeddings between generation~\cite{zhang2020bertscoreevaluatingtextgeneration} and context/reference.
Based on the ways of measuring embedding similarity, existing embedding-based evaluation methods can be classified into following three categories: (1) Cosine Similarity; (2) Embedding Distance; (3) Divergence.

\textbf{Cosine similarity} are the most widely used method for measuring the semantic similarity of text embeddings~\cite{zhao-etal-2023-discoscore,su-etal-2023-one,10079300,akula-garibay-2022-sentence,10.1145/3459637.3482463,lo-2019-yisi,mathur-etal-2019-putting,liu-etal-2023-revisiting-commonsense,koto-etal-2021-evaluating,zhan-etal-2021-difficulty,gao-etal-2020-supert,chen-guo-2015-representation,odonoghue-etal-2023-bioplanner,bansal-etal-2022-sem}.
Prior to pre-trained language models like BERT~\cite{devlin-etal-2019-bert}, most studies typically employed word embeddings to construct  semantic vectors for text~\cite{ng-abrecht-2015-better,sun-nenkova-2019-feasibility}, like Word2Vec~\cite{mikolov2013efficientestimationwordrepresentations} and GloVe~\cite{pennington-etal-2014-glove}. 
For example, Vector Extrema, Embedding Average, Greedy Matching \cite{liu-etal-2016-evaluate} leverage cosine similarity to evaluate the quality of dialog generation.
With the emergence of pre-trained language models (PLMs) represented by BERT~\cite{devlin-etal-2019-bert} and RoBERTa~\cite{liu2020roberta}, semantic embedding generated by PLMs have been proven to capture semantic information more effectively, resulting in more robust embedding-based evaluation methods~\cite{chen-etal-2021-training,zhao-etal-2020-limitations,li-etal-2021-conversations,zhu-etal-2023-imagine,zhou-etal-2023-codebertscore}. BERTScore~\cite{Zhang2020BERTScore:} is the most representative embedding-based, using pre-trained BERT model as backbone. 
It first leverages the BERT model for obtaining semantic vectors, and computes the IDF-weighted maximum cosine similarity between each pair of reference and generation token.

\textbf{Word Mover's Distance} is also widely used for embedding-based methods \cite{zhao-etal-2019-moverscore,clark-etal-2019-sentence,colombo-etal-2021-automatic,song-etal-2021-sentsim,ijcai2020p516,pmlr-v37-kusnerb15,chow-etal-2019-wmdo}, where lower distance denotes the close performance of generations to references. The most widely-used distance is the euclidean distance and $\mathcal{L}_p$ distance, where $p\in \{1,2,+\infty\}$. For example, MoverScore \cite{zhao-etal-2019-moverscore} computes the word mover distance (euclidean distance) between generations and references, by using the BERT as the embedding model. WMD~\cite{pmlr-v37-kusnerb15} and Sentence Mover’s Similarity (SMS) \cite{clark-etal-2019-sentence} measures the cost of moving generations to references using semantic embeddings. \citet{xiang-etal-2021-assessing} leverages the Frechet Bert Distance (FBD) to compute the distance between references and generations.

\textbf{Divergence} is another embedding-based evaluation metrics. For example, InfoLM \cite{Colombo2021InfoLMAN}  uses different kinds of divergences to comparing two well formed discrete probability distributions of references and generations. MAUVE \cite{NEURIPS2021_260c2432} measures the KL-divergence between the references and generations by using their mixture distribution.



\input{latex/sections/table_eval_metric_learning_based}



\subsubsection{Learning-based Evaluation}
Embedding-based evaluation methods struggle to achieve strong consistency with human judgments because of two reasons:
(1) Since text embeddings only capture the semantic information of the generations, neglecting some severe error patterns, such as  grammar correctness and diversity;
(2) the limited number of reference or context could not cover all the high-quality candidates in the open-domain generation tasks. Therefore, it is easy to misjudge high-quality generations that are not similar to the given reference or context.
Inspired by data-driven machine learning methods, numerous works attempt to optimize deep neural networks to imitate how human annotators evaluate the quality of generations~\cite{lowe-etal-2017-towards}, leading to a new paradigm of evaluation metrics, \textit{i.e.}, \textbf{\textcircled{\scriptsize{3}}} \textbf{\textit{Learning-based Evaluation}}.
Through optimizing on the established datasets for text evaluation, learning-based automatic evaluation methods captures the features about judging the quality of generations. 
So far, Based on the different approaches to construct evaluation dataset, existing automatic evaluation metrics can be classified into the following three categories: 
(1) \textbf{Supervised} leverages the human-annotated evaluation datasets to optimize the learning-based evaluation methods;
% TODO: 说明和LLM-based fine-tuning-based中使用GPT-4自动构建的区别
(2) \textbf{Self-supervised} synthesize the flawed generations given the high-quality references for training the evaluation models;
(3) \textbf{Mixture} method first pre-trained the evaluation models on large-scale self-supervised datasets, and then fine-tuned them on the high-quality human-annotated supervised dataset.

\paragraph{Supervised}


Supervised learning-based automatic evaluation methods optimize models to simulate human assessment by training on high-quality manually annotated scoring data $(c^*,cri^*,r^*,g,s)$~\cite{mathur-etal-2019-putting,Zhang2021,weston-etal-2022-generative,sellam-etal-2020-bleurt,liu-etal-2023-towards-interpretable,pu-etal-2021-learning,rubino-etal-2021-error,bulian-etal-2022-tomayto,wang-etal-2022-paratag}.
So far, based on the need of reference $r$ and context $c$, most of supervised learning-based evaluation methods could be classified into four categories: (1) reference-based and context-free; (2) reference-based and context-based; (3) reference-free and context-free; (4) reference-free and context-based.

Early reference-based and context-free supervised methods usually fine-tune the hyper-parameter or train a pairwise classifier a regressions based on the RNN/LSTM model \cite{guzman-etal-2015-pairwise,guzman-etal-2014-learning,gupta-etal-2015-reval}. For example, Q-BLEU4 \cite{nema-khapra-2018-towards} tunes two hyper-parameters on human-annotated scores that incorporates the answerbilitiy score and BLEU-4 scores for automatic question generation (AQG) system. RUSE \cite{shimanaka-etal-2018-ruse} is a regression model trained on the human-annotated translation quality scores. ADEM \cite{lowe-etal-2017-towards} optimizes RNN models for evaluating the quality of generated dialog utterance based on the conversation history and the reference utterance.

Reference-based and context-based methods evaluate the generation by considering both reference and context information.
The most representative methods COMET~\cite{rei-etal-2020-comet}, which designs two variants\textemdash COMET-MQM and COMET-DARR that trained on the human-annotated machine translation corpus, considering the source sentence, and human-generated reference translations. 
\citet{takahashi-etal-2020-automatic} also trained a Similar machine translation evaluation methods based on the XLM model \cite{lample2019crosslingual}.
The reference-based and context-based methods are also applied in other NLG tasks. For example, as for text simplication task, LENS \cite{maddela-etal-2023-lens}, a learnable metrics trained on human-annotated text, outperforms strong baselines like BERTScore.
RADE \cite{shi-etal-2023-rade} also evaluate the quality scores of dialog generations with human-generated responses as references.
Furthermore, LERC \cite{chen-etal-2020-mocha} is trained on human judgments in its annotated MOCHA dataset of Generative Reading Comprehension task.

Reference-free and context-based supervised methods are widely used for the open-domain dialogue generation, which primilary evaluates the coherence with the context. 
DialogRPT \cite{gao-etal-2020-dialogue} optimize the DialoGPT \cite{zhang2020dialogptlargescalegenerativepretraining} model on the human-annotated rating datasets to train the ranking model as the learnable metric.
DEB \cite{sai-etal-2020-improving} construct a high-quality human-annotated datasets for training dialogue response evaluation model, consisting of multiple references and adversarial responses.

Reference-free and context-free supervised method is a very special supervised learning-based evaluation methods, which usually focus on the open-domain open-domain generation with less constraints of the context.
For instance, SLE \cite{cripwell-etal-2023-simplicity}, StoryER \cite{chen-etal-2022-storyer} and ASE-Eval \cite{taghipour-ng-2016-neural} are designed for text simplification, story generation and  Automated Essay Scoring (ASE), specifically, trained on Newsela dataset \cite{10.1162/tacl_a_00139}.



\paragraph{Self-supervised}

Since the collection of human-annotated evaluation datasets is expensive, numerous works are proposed to automatically construct the evaluation dataset by designing negative sampling strategy~\cite{jwalapuram-etal-2019-evaluating}
%\footnote{Recently, there is a emerging trend to automatically synthetic datasets by using state-of-the-art teacher model, like GPT-4. Since most of these datasets are not annotated by human annotators, it is also a self-supervised method. However, in this section, we mainly discuss the prior learning-based automatic evaluation methods that are proposed before the concept of the LLMs (THE DATE OF THE LLM/CHATGPT). Please refer to Section~\ref{} for more details about related works in data synthesis of teacher model like GPT-4.}
, such as negative sampling~\cite{tao2017ruberunsupervisedmethodautomatic} and data synthesis~\cite{zhang2022mddevalselftrainingaugmenteddata,lan2020ponenovelautomaticevaluation}.
Based on the used strategies for generating the self-supervised training datasets, existing self-supervised learning-based evaluation methods could be classified into four categories: (1) text perturbation; (2) generative augmentation; (3) negative sampling; and (4) positive augmentation.

\textbf{Text perturbation} is the most widely used strategy to construct the negative samples for training~\cite{phy-etal-2020-deconstruct,rony-etal-2022-rome,guan-huang-2020-union}. For example, DENSITY~\cite{park-etal-2023-density}, ReFreeEval~\cite{wu-etal-2023-holistic}, LS Score~\cite{wu-etal-2020-unsupervised} and \textsc{UniEval}~\cite{zhong-etal-2022-towards} apply the random-span repetition, insertion, deletion, substitution and disorder operations to construct the high-quality references to generate the low-quality generation with flaws. Except for these operations, UNION~\cite{guan-huang-2020-union} also introduce the negation aleartion for story generation task. Besides, MDD-Eval~\cite{zhang2022mddevalselftrainingaugmenteddata} and PoE~\cite{10056996} also leverage the back-translation to generate fluent but flawed generations. The mask-and-fill operation is also widely used to corrupt the reference answer~\cite{zhang2022mddevalselftrainingaugmenteddata,lu2022humanlikeevaluationnaturallanguage}.

\textbf{Negative sampling} is another widely used strategy, which construct negative samples by randomly sampling them from the corpus~\cite{tao2017ruberunsupervisedmethodautomatic,mehri-eskenazi-2020-unsupervised,ghazarian-etal-2019-better}. For example, RUBER~\cite{tao2017ruberunsupervisedmethodautomatic} randomly samples dialogue utterances from the corpus to form the negative samples for each user query. Since random negative samples are easy to distinguish, numerous works recognize the importance of high-quality negative sampling and design some hard negative sampling strategy~\cite{xu-etal-2023-sescore2,zhang-etal-2022-fined,zhang-etal-2021-dynaeval,lan2020ponenovelautomaticevaluation,zhou2020learningcomparebettertraining,10.1109/TASLP.2021.3074012}. For example, PoNe~\cite{lan2020ponenovelautomaticevaluation} selects the negative samples with higher semantic similar with conversation context, while GRADE~\cite{huang-etal-2020-grade} select utterances with higher similarity with reference answers.

\textbf{Generative Augmentation} leverages the pre-trained language models (PLMs) to generate fluent while inappropriate negative samples for evaluation. For example, PoNe and MDD-Eval leverage the Seq2Seq~\cite{vaswani2017attention} and DialoGPT~\cite{zhang2019dialogpt} model to construct evaluation datasets.

\textbf{Positive Augmentation} aims to construct the positive samples for evaluation, rather than the negative samples in above three methods~\cite{lan2020ponenovelautomaticevaluation,zhang2022mddevalselftrainingaugmenteddata}. For example, PoNe~\cite{lan2020ponenovelautomaticevaluation} observes that the unbalanced positive and negative data distribution significantly influence the robustness of the learning-based methods, and propose to supplement positive samples to balance the training dataset.

However, the false negative samples significantly influence the quality of established self-supervised datasets. For example, the generative augmentation usually provides fluent and appropriate samples, and hard negative sampling also have chance to select the appropriate and coherent dialogue utterance. To overcome this problem, numerous works~\cite{lan2020ponenovelautomaticevaluation,zhang2022mddevalselftrainingaugmenteddata,10056996} propose the pseudo labeling methods to detect and remove these false negative samples.



\paragraph{Mixture}
Models trained through supervised learning typically perform better than self-supervised methods due to the benefits of high-quality manually annotated data. However, self-supervised methods can quickly construct large-scale evaluation datasets without expensive manual annotation costs, thereby improving the performance of evaluation models. Therefore, combining the advantages of both methods is also a viable technical solution. 
For example, BLEURT~\cite{sellam-etal-2020-bleurt}, FrugalScore \cite{kamal-eddine-etal-2022-frugalscore} and MisMATCH \cite{murugesan-etal-2023-mismatch} first pre-trained a BERT model on vast synthetic reference-candidate pairs, and then fine-tune it on the human-annotated scores. 




% 和critic的关系也要阐述
\subsubsection{LLM-based Evaluation}
\label{sec:llm_based_evaluation}


Learning-based methods heavily rely on high-quality and diverse training samples. It is a challenge to generalize the trained learning-based methods to out-of-domain tasks and evaluation criteria. 
Due to the advanced instruction following, context understanding and zero-shot generalization ability of the emerged large-scale language models (LLMs), there is an increasing trend to implement automatic evaluation models built on LLMs, resulting in the \textbf{\textcircled{\scriptsize{4}}} \textbf{\textit{LLM-based Evaluation}}, which is also known as the concept of LLM-as-a-judge~\cite{li2024generationjudgmentopportunitieschallenges}.
Compared to previous heuristic, embedding-based and learning-based automatic evaluation, LLM-based evaluation could not only provide the evaluation judgment but also the textual rationale to analyze the flaws in generations and rise some valuable revision suggestions, resulting in more fine-grained and better interpretable evaluations.
So far, existing LLM-based evaluation methods can be classified into two categories: (1) Prompt-based methods designs the evaluation guidelines in the prompt to ask LLMs play as an annotator; (2) Fine-tuning-based methods try to improve the evaluation capability of efficient LLMs with small-paramters, addressing the huge budget of inferencing the expensive LLMs, like GPT-4, which is also known as the reward model in recent LLMs alignment researches~\cite{ouyang2022traininglanguagemodelsfollow}.

\paragraph{Prompt-based Methods}



Through simply designing the prompts, LLMs could effectively handle the evaluation tasks across diverse NLG tasks and evaluation criteria~\cite{fu2023gptscoreevaluatedesire,lin-chen-2023-llm}. For example, \citet{wang2023chatgptgoodnlgevaluator} and \citet{liu2023gevalnlgevaluationusing} demonstrate that GPT-3.5 and GPT-4 are the good zero-shot evaluator for diverse NLG tasks.
Building upon these works, numerous works have proposed various techniques to further improve the robustness of the LLM's evaluation capabilities:
% reference
(1) \textbf{Reference:} \citet{zheng2023judgingllmasajudgemtbenchchatbot} and \citet{badshah2024referenceguidedverdictllmsasjudgesautomatic} evaluate the quality of response by comparing it with the reference response;
% criteria
(2) \textbf{Criteria:} \citet{qian-etal-2024-large,kim2024prometheus2opensource,lu2024exactmatchsemanticallyreassessing} provide detailed evaluation criteria and rubrics to guide LLMs's evaluation;
% demonstration
(3) \textbf{Demonstration:} Besides, GPTScore~\cite{fu2023gptscoreevaluatedesire}, ICE~\cite{jain-etal-2023-multi}, MSoR~\cite{song2025manyshotincontextlearninghelp}
, Little Giants~\cite{kotonya-etal-2023-little} and ALLURE~\cite{hasanbeig2023allureauditingimprovingllmbased} augments the LLM-based evaluation by providing the few-shot demonstrations;
% positionalswapping for consistency
(4) \textbf{Swapping:} Additionally, the swapping operations are widely used to reduce the positional bias for pair-wise evaluation~\cite{lan2024criticevalevaluatinglargelanguage,lee2024rlaifvsrlhfscaling,zheng2023judgingllmasajudgemtbenchchatbot};
% self-consistency
(5) \textbf{Self-consistency:} Moreover, \citet{zhang2024selfcontrastbetterreflectioninconsistent,zheng2023judgingllmasajudgemtbenchchatbot} notice that LLM-as-a-judge could be improved by using self-consistency prompting strategy, which samples multiple evaluation rationale and conduct the majority voting as the final evaluation result;
% multi-agent
(6) \textbf{Multi-Agent:} Furthermore, recognizing the significant of the single-model bias during evaluation, numerous works also design the multi-agent debate framework for evaluation task, such as ChatEval~\cite{chan2023chatevalbetterllmbasedevaluators}, PoLL~\cite{verga2024replacingjudgesjuriesevaluating} and PRD~\cite{li2024prdpeerrankdiscussion}.

%%% 
In summary, most prompt-based methods described above propose the prompting strategies to reduce the inconsistency of the LLMs\textemdash generating inconsistent responses by LLMs~\cite{liang2024internalconsistencyselffeedbacklarge,zhang2024selfcontrastbetterreflectioninconsistent,wang2023selfconsistency}. % 介绍一下 inconsisteny 的含义，以及我们怎么把已有的工作和这个内容联系起来。
For example, LLMs could achieve more accurate judgments on the quality of evaluated response by following the guidelines and clues provided in demonstration, detailed criteria and reference response. Besides, self-consistency and multi-agent are also widely used to reduce the inconsistency and bias of one single model.



\paragraph{Fine-tuning-based Methods}

Due to the expensive cost of inference LLMs with large volume of parameters for evaluation, numerous works propose to fine-tune the efficient LLMs to improve their evaluation capabilities, leading to the fine-tuning-based evaluation methods. The efficient LLMs for evaluation models not only address the huge requirements for large-scale evaluation, but also serve as the reward models in RLHF training phase~\cite{mahan2024generativerewardmodels,lee2024rlaifvsrlhfscaling,ouyang2022traininglanguagemodelsfollow}.
Currently, existing fine-tuning-based LLM evaluation methods can be classified along three dimensions~\cite{zeng2024scalingsearchlearningroadmap,li-etal-2024-leveraging-large}: 
(1) \textbf{Evaluation Granularity:} early evaluation granularity is the whole response, or outcome-based reward models (ORMs) or evaluation models,~\cite{lightman2023letsverifystepstep}, while recent works~\cite{zeng2024scalingsearchlearningroadmap} recognize that fine-grained and dense process reward models (PRMs) leads to better transpancy and effective feedback, with the cost of high human-labor for annotating process reward signals~\cite{lightman2023letsverifystepstep}.; 
(2) \textbf{Optimization Methods:} supervised fine-tuning (SFT) is the most widely-used way to improve the evaluation capabilities of LLMs~\cite{li2023generativejudgeevaluatingalignment,cui2023ultrafeedback}. Recently, numerous works begin to improve the evaluation capabilities of LLMs by using preference learning techniques, like DPO~\cite{rafailov2024directpreferenceoptimizationlanguage} or RL~\cite{ouyang2022traininglanguagemodelsfollow}, aiming to address the limitations of the behavior cloning; 
and (3) \textbf{Data Sources:} the datasets for optimizing the evaluation abilities of LLMs are from three sources: (a) the advanced teacher model like GPT-4; and (b) human experts; (c) human-model interaction where models generate evaluation dataset which are filtered by comparing model judgments with human annotation. Although the teacher model could generate large-scale datasets in a scalable way, the quality of their dataset falls significantly short compared to human annotation.
The representative fine-tuning-based LLM-based evaluation methods are listed in Table~\ref{tab:fine_tuning_llm_evaluation}, and we will discuss some of them from following aspects: evaluation granularity, optimization, and data source.

\input{latex/sections/table_eval_metric_llm_based}

Shepherd~\cite{wang2023shepherd} asks human experts to annotate textual evaluation samples for training Llama-7B. 
Due to the huge budget of annotating textual evaluations, numerous work leverages the advanced teacher model like GPT-4 to construct the pseudo samples for training, like Auto-J~\cite{li2024generationjudgmentopportunitieschallenges} and UltraCM~\cite{cui2023ultrafeedback}.
However, these model-generated datasets contains lots of noises that may affect the robustness of trained evaluation models. Therefore, some works propose to sample numerous draft samples and filter the high-quality samples by using human-annotated scalar scores.
For example, Themis~\cite{hu2024themisreferencefreenlgevaluation} and SFR~\cite{wang2024directjudgementpreferenceoptimization} filters high-quality GPT-4 generated samples by computing the consistency between GPT-4's judgment and human judgments.

Early works usually optimize the LLMs on evaluation corpus using SFT~\cite{li2024generationjudgmentopportunitieschallenges,xu-etal-2023-instructscore,wang2023shepherd,kim2024prometheus2opensource}. Recent works recognize that performance of evaluation models is limited by the quality of supervised dataset during SFT training phase. Therefore, numerous works propose to improve the evalutaion model by leveraging preference learning techniques, like DPO~\cite{trivedi2024selfrationalizationimprovesllmfinegrained,yu2024selfgeneratedcritiquesboostreward,wang2024directjudgementpreferenceoptimization} and RL~\cite{lan2024traininglanguagemodelscritique}. 

Most fine-tuning-based evaluation models are outcome-based, which evaluate the correctness of the response as a whole~\cite{cui2023ultrafeedback,kim2024prometheus2opensource}. 
In order to achieve better transparency and explanation, some works locate the fine-grained flaws in responses and propose detailed analysis about them, such as InstructScore~\cite{xu-etal-2023-instructscore}, TIGERScore~\cite{jiang2024tigerscorebuildingexplainablemetric} and MultiCritique~\cite{lan2024traininglanguagemodelscritique}.
Even so, evaluation signals still remain sparse as there aren't many flaws in the responses.
Recently, there is an emerging trend to provide more dense evaluation signals for all intermediate steps in the responses, also known as the process-based reward models (PRMs). For example, \citet{lightman2023letsverifystepstep} annotate the correctness of each intermediate rationale in solving the mathematic solutions.
While the PRMs could provide dense and fine-grained feedback information, it is much more expensive and difficult to annotate intermediate steps than the whole response.
Therefore, lots of works employ Monte Carlo Tree Search (MCTS) to construct the process signals automatically in the reasoning tasks with human-annotated ground-truth answers, such as Math-Shepherd~\cite{wang-etal-2024-math} and xxx.


\subsubsection{Benchmark-based Evaluation}

Beyond designing automatic evaluation methods, there exists a distinct category we call benchmark evaluation. This method primarily assess the consistency between NLG models and human annotations on pairs of questions and human-annotated answers, thereby measuring the general capability of NLG models. 
Since manual annotation is completed as a one-time effort, subsequent model evaluations only require simple verification of the match between NLG model-generated answers and human annotations, which could be simple answer verification, exact matching, and automatic evaluations we described in previous Sections.

As shown in Table~\ref{tab:benchmark_evaluation}, existing benchmarks can be categorized into the following types~\cite{2023opencompass} based on the different capabilities being evaluated: 
(1) \textbf{Knowledge} evaluates the general or doman-specific knowledge capacity of NLG models~\cite{huang2023ceval}. For example, C-Eval~\cite{huang2023ceval} evaluates the STEM, Humanities and Social Science knowledges capacity of LLMs, and MedBench evaluates LLM's capability in the medical domain; 
(2) \textbf{Reasoning} evaluates the logic reasoning capability of NLG models under some reasoning tasks, like mathematics~\cite{cobbe2021gsm8k} and coding tasks\cite{chen-etal-2021-training}. 
(3) \textbf{Understanding} evaluates the capabilities of NLG models or LLMs in understanding the purpose of the context or user queries, such as MT-Bench101~\cite{bai2024mt} and XSum~\cite{narayan2018dont}; 
(4) \textbf{Long Text} aims to evaluate the long context modeling capability of LLMs, such as LongBench~\cite{bai2023longbench} and Ada-LEval~\cite{wang2024adaleval}; 
(5) \textbf{Agent} evaluates LLMs in automatic task solving, function calling tasks capabilities~\cite{chen2023t,ma2024agentboard}; 
(6) \textbf{Instruction-Following} evaluates whether the LLMs strictly follow the user's instruction or align with human desires, like IFEval~\cite{zhou2023instruction}.

\input{latex/sections/table_benchmarks}


\subsection{Meta-Evaluation Benchmarks}
\label{sec:meta_evaluation_benchmarks}
As shown in Table~\ref{tab:meta_evaluation_benchmarks}, there are numerous meta-evaluation benchmarks are proposed to measure the reliability of automatic evaluations. 
Early meta-evaluation benchmarks mainly focus on specific NLG tasks, such as machine translation~\cite{freitag-etal-2022-results,fu2023gptscoreevaluatedesire}, text summarization~\cite{fabbri2021summeval,Bhandari-2020-reevaluating,grusky-etal-2018-newsroom}, data-to-text generation~\cite{mairesse-etal-2010-phrase,wen-etal-2015-semantically,zhou-lampouras-2020-webnlg,lin-etal-2020-commongen}, open-domain dialog generation~\cite{mehri-eskenazi-2020-unsupervised,mehri-eskenazi-2020-usr}, and story generation~\cite{guan-etal-2021-openmeva,wang-etal-2022-paratag}.
Given the advanced generation and generalization ability of LLMs, numerous general meta-evaluation benchmarks are proposed to systematically evaluate their evaluation capability in diverse and general domains, such as MT-Bench, Chat Arena~\cite{zheng2023judging} and RewardBench~\cite{lambert2024rewardbenchevaluatingrewardmodels}.
Besides, some meta-evaluation benchmarks also focus on measuring the evaluation ability of LLMs in some challenging tasks, such as reasoning tasks~\cite{luo2023critiqueabilitylargelanguage,lin-etal-2024-criticbench,tan2024judgebenchbenchmarkevaluatingllmbased}, safety alignment~\cite{yuan2024rjudgebenchmarkingsafetyrisk} and information retrieval~\cite{lu2024exactmatchsemanticallyreassessing}.

\input{latex/sections/table_meta_evaluation}


%\subsection{Trends in Paradigms Shift}
\subsection{Challenges \& Future Works of NLG Automatic Evaluation}
\label{sec:conclusion_challenge_future}

In this section, we elaborate the current challenges and promising research directions for NLG automatic evaluation, including Evaluation Bias~\ref{}, Flexible Evaluation Criteria~\ref{}, Efficient Automatic Evaluation~\ref{}, and 

\subsubsection{Bias and Inconsistency of Automatic Evaluation}

%%% bias
Although LLM-based evaluation is the most advanced automatic evaluation method, they suffer from the bias brought from their large-scale pre-trained data~\cite{li2024generationjudgmentopportunitieschallenges,li-etal-2024-leveraging-large,ye2024justiceprejudicequantifyingbiases}. 
For example, ~\citet{ye2024justiceprejudicequantifyingbiases} highlights 12 key potential bias during using LLM-based evaluation methods.
%%% consistency
%%%% refer to paper: https://arxiv.org/abs/2405.01724, https://arxiv.org/html/2406.00231v2
Except for these evaluation bias, recent works also demonstrate that LLM-based evaluations would generate inconsistent evaluations with multiple evaluations~\cite{stureborg2024largelanguagemodelsinconsistent,zeng2024llmrankfusionmitigatingintrinsicinconsistency}. For example, the ``inter-sample'' agreement of LLMs is much lower than human-annotators, indicating that LLMs could provide inconsistent evaluations during multiple inferences.
These bias and inconsistency significantly hinders the deployment of these LLM-based evaluation methods in the diverse real-world scenarios.

%%% future works
\paragraph{Future Work.} 

Although self-consistency may be an effective way to solve the inconsistency of LLM-based evaluation methods, its large inference budget is unbearbale during deployment. Therefore, future works 

\subsubsection{Generalization of Automatic Evaluation}

The evolution of automatic evaluation techniques of NLG has led to significant improvements in the generalization of evaluation methods. 
Early automatic evaluation approaches typically designed task-specific evaluation methods around particular evaluation criteria~\cite{fu2023gptscoreevaluatedesire,li-etal-2024-leveraging-large}. For instance, early heuristic evaluation, embedding-based metrics and learning-based evaluation methods assessed the specific evaluation criteria such as semantic coverage, coherence, fluency~\cite{fu2023gptscoreevaluatedesire}.

Recent LLM-based evaluation methods have exhibited remarkable flexibility and generalization~\cite{fu2023gptscoreevaluatedesire}, enabling dynamic and adaptable evaluation by simply designing evaluation criteria within prompts.

\paragraph{Future Direction}
%%% TODO: https://aclanthology.org/2024.lrec-main.237.pdf
However, it is noteworthy that trained automatic evaluation methods (whether learning-based or fine-tuned-based LLM-based) tend to compromise their evaluation generalization, particularly for domains and evaluation criteria that not covered in the training data. 
Existing learning-based or LLM-based (fine-tuned-based) automatic evaluation methods rely on models to implicitly learn evaluation criteria of specific tasks, which not only increases the complexity of evaluation but also reduces generalization. 
Therefore, explicit learning of evaluation criteria represents a crucial direction for future development, which has been explored recently.
For example, HD-Eval~\cite{liu2024hdevalaligninglargelanguage} learns to construct a hierarchical criteria tree using human-annotation labels, and prove this criteria structure could further improve the LLM-based evaluation methods, like G-Eval~\cite{liu2023gevalnlgevaluationusing}.
Besides, MultiCritique~\cite{lan2024traininglanguagemodelscritique} jointly learns customized criteria and evaluation generation within a multi-task learning framework, significantly enhancing evaluation generalization.





\subsubsection{From Outcome-based to Process-based Automatic Evaluation}

The rapid advancement of strong reasoning models like OpenAI-o1 highlights the significance of process-based reward models (evaluation models). However, process-based evaluation models heavily depend on high-quality human-annotated datasets~\cite{lightman2023letsverifystepstep}. While methods like MCTS can currently synthesize process evaluation labels for reasoning tasks with definitive answers~\cite{zeng2024scalingsearchlearningroadmap}, such as coding and mathematical problems, constructing process-based evaluation data in open-domain scenarios remains an unexplored research area.
\paragraph{Future Direction} should focus on how to construct the general process-based annotation datasets for all kinds of task scenarios, except for the reasoning tasks.

\subsubsection{Application of Automatic Evaluation}

In the era of large language models, beyond alleviating or eliminating costly human evaluation, automatic evaluation techniques play indispensable roles in two key areas~\cite{lan2024traininglanguagemodelscritique,lan2024criticevalevaluatinglargelanguage}: 
(1) \textbf{Self-improvement of LLMs}: numerous studies explore utilizing LLMs' automatic evaluation capabilities to synthesize high-quality data for enhancing language model performance. For example, self-rewarding~\cite{yuan2024selfrewardinglanguagemodels} constructs the preference datasets annotated by the optimized LLM itself, and iteratively improve the alignment of the LLM.
Unlike Themis~\cite{hu2024themisreferencefreenlgevaluation}, SFR~\cite{wang2024directjudgementpreferenceoptimization} and Critic-RM~\cite{yu2024selfgeneratedcritiquesboostreward} that leverages human-annotated labels as ground-truth to synthesize dataset, these methods eliminates the dependency on human annotations, enabling efficient self-improvement of LLM capabilities;
(2) \textbf{Robust RLHF}: recently, numerous works have recognized the potential of generative reward models or LLM-based evaluation method~\cite{mahan2024generativerewardmodels,ye2024improvingrewardmodelssynthetic,ankner2024critiqueoutloudrewardmodels}.
Besides, DeepSeek-V3~\cite{deepseekai2024deepseekv3technicalreport} also leverages the generative reward models to provide accurate reward signal during reinforcement learning phase.

\paragraph{Future Directions} of these two important applications of automatic evaluations are described as follows:
(1) \textbf{Self-improvement of LLMs}: While self-improvement shows great promise, recent studies indicate that its upper bound is constrained by the performance of the evaluation capability of LLM itself~\cite{wu2024metarewardinglanguagemodelsselfimproving}. 
Although meta-rewarding~\cite{wu2024metarewardinglanguagemodelsselfimproving} implements two rounds of DPO optimization to improve both generation and evaluation capabilities simultaneously, the upper bound of self-improvement is still limited by the evaluation capability. 
Future work should explore more effective methods to enhance evaluation capabilities and accelerate LLM's self-improvement, such as adopting multi-agent frameworks~\cite{lan2024traininglanguagemodelscritique} or incorporating minimal human annotations to reduce bias~\cite{ye2024improvingrewardmodelssynthetic};
(2) \textbf{Robust RLHF}: Although generative reward models significantly outperform traditional reward models in accuracy, they require generating rationale chains-of-thought for reasoning and analysis before producing final reward signals, which further intensifies the computational burden of the RLHF training phase. Therefore, future work should focus on how to effectively distill evaluation capabilities into efficient generative reward models, which has been detailed in Section~\ref{sec:llm-based-fine-tuned-based}.


%% related self-judging
\subsubsection{Source of Training Data of Automatic Evaluation}

Improving the evaluation capabilities of efficient models through training, \textit{i.e.} fine-tuned-based LLM-based evaluation, represents a significant development trend. Currently, evaluation data primarily originates from either powerful teacher models like GPT-4~\cite{li2023generativejudgeevaluatingalignment,cui2023ultrafeedback} or human annotations~\cite{wang2023shepherd,ye2024improvingrewardmodelssynthetic,hu2024themisreferencefreenlgevaluation}. However, as tasks become increasingly complex, neither individual teacher models nor human experts can provide reliable supervision signals to further enhance automated models. 

\paragraph{Future Direction} Therefore, in the future, it is an important direction to aggregate multi-agent evaluation capabilities to improve the reliability of automatic evaluation techniques. For example, ChatEval~\cite{}, PoLL~\cite{verga2024replacingjudgesjuriesevaluating} and Stable Alignment~\cite{liu2023sociallyaligned} improves the evaluation and generation capabilities of LLMs through learning from multi-agent discussion and social interaction.



==> sections/AE/ae_nlg_subsections/limitation.tex <==
\paragraph{Limitation of Challenges and Future Works}

Due to the page limitation, we do not dedicate much content to discussing the challenges and future directions of automated evaluation for NLG. 
Instead, the primary goal of this paper is to summarize and analyze existing paradigms of automated evaluation techniques and, based on this foundation, extend the analysis to automated evaluation methods in the vision and speech modalities.

%%%%%%%%%%%%%%%%
\iffalse
\subsection{Challenges \& Future Works of NLG Automatic Evaluation}
\label{sec:conclusion_challenge_future}

In this section, we elaborate the current challenges and promising research directions for NLG automatic evaluation, including Evaluation Bias~\ref{}, Flexible Evaluation Criteria~\ref{}, Efficient Automatic Evaluation~\ref{}, and 

\subsubsection{Bias and Inconsistency of Automatic Evaluation}

%%% bias
Although LLM-based evaluation is the most advanced automatic evaluation method, they suffer from the bias brought from their large-scale pre-trained data~\cite{li2024generationjudgmentopportunitieschallenges,li-etal-2024-leveraging-large,ye2024justiceprejudicequantifyingbiases}. 
For example, ~\citet{ye2024justiceprejudicequantifyingbiases} highlights 12 key potential bias during using LLM-based evaluation methods.
%%% consistency
%%%% refer to paper: https://arxiv.org/abs/2405.01724, https://arxiv.org/html/2406.00231v2
Except for these evaluation bias, recent works also demonstrate that LLM-based evaluations would generate inconsistent evaluations with multiple evaluations~\cite{stureborg2024largelanguagemodelsinconsistent,zeng2024llmrankfusionmitigatingintrinsicinconsistency}. For example, the ``inter-sample'' agreement of LLMs is much lower than human-annotators, indicating that LLMs could provide inconsistent evaluations during multiple inferences.
These bias and inconsistency significantly hinders the deployment of these LLM-based evaluation methods in the diverse real-world scenarios.

%%% future works
\paragraph{Future Work.} 

Although self-consistency may be an effective way to solve the inconsistency of LLM-based evaluation methods, its large inference budget is unbearbale during deployment. Therefore, future works 

\subsubsection{Application of Automatic Evaluation}

In the era of large language models, beyond alleviating or eliminating costly human evaluation, automatic evaluation techniques play indispensable roles in two key areas~\cite{lan2024traininglanguagemodelscritique,lan2024criticevalevaluatinglargelanguage}: 
(1) \textbf{Self-improvement of LLMs}: numerous studies explore utilizing LLMs' automatic evaluation capabilities to synthesize high-quality data for enhancing language model performance. For example, self-rewarding~\cite{yuan2024selfrewardinglanguagemodels} constructs the preference datasets annotated by the optimized LLM itself, and iteratively improve the alignment of the LLM.
Unlike Themis~\cite{hu2024themisreferencefreenlgevaluation}, SFR~\cite{wang2024directjudgementpreferenceoptimization} and Critic-RM~\cite{yu2024selfgeneratedcritiquesboostreward} that leverages human-annotated labels as ground-truth to synthesize dataset, these methods eliminates the dependency on human annotations, enabling efficient self-improvement of LLM capabilities;
(2) \textbf{Robust RLHF}: recently, numerous works have recognized the potential of generative reward models or LLM-based evaluation method~\cite{mahan2024generativerewardmodels,ye2024improvingrewardmodelssynthetic,ankner2024critiqueoutloudrewardmodels}.
Besides, DeepSeek-V3~\cite{deepseekai2024deepseekv3technicalreport} also leverages the generative reward models to provide accurate reward signal during reinforcement learning phase.

\paragraph{Future Directions} of these two important applications of automatic evaluations are described as follows:
(1) \textbf{Self-improvement of LLMs}: While self-improvement shows great promise, recent studies indicate that its upper bound is constrained by the performance of the evaluation capability of LLM itself~\cite{wu2024metarewardinglanguagemodelsselfimproving}. 
Although meta-rewarding~\cite{wu2024metarewardinglanguagemodelsselfimproving} implements two rounds of DPO optimization to improve both generation and evaluation capabilities simultaneously, the upper bound of self-improvement is still limited by the evaluation capability. 
Future work should explore more effective methods to enhance evaluation capabilities and accelerate LLM's self-improvement, such as adopting multi-agent frameworks~\cite{lan2024traininglanguagemodelscritique} or incorporating minimal human annotations to reduce bias~\cite{ye2024improvingrewardmodelssynthetic};
(2) \textbf{Robust RLHF}: Although generative reward models significantly outperform traditional reward models in accuracy, they require generating rationale chains-of-thought for reasoning and analysis before producing final reward signals, which further intensifies the computational burden of the RLHF training phase. Therefore, future work should focus on how to effectively distill evaluation capabilities into efficient generative reward models, which has been detailed in Section~\ref{sec:llm-based-fine-tuned-based}.

\fi
%
